Analysing the Complexity of Functional Programs: Higher-Order Meets First-Order (Long Version)

We show how the complexity of higher-order functional programs can be analysed automatically by applying program transformations to a defunctionalized versions of them, and feeding the result to existing tools for the complexity analysis of first-order term rewrite systems. This is done while carefully analysing complexity preservation and reflection of the employed transformations such that the complexity of the obtained term rewrite system reflects on the complexity of the initial program. Further, we describe suitable strategies for the application of the studied transformations and provide ample experimental data for assessing the viability of our method.

==> conclusion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusion}
%%%%%%%%%%%%%%%%%%%%%%%
We have shown how complexity analysis of higher-order functional
programs can be reduced to defunctionalization, followed by other
program transformations which do not perform any complexity analysis,
but whose role consists in putting the program into a form suitable to
the analysis by existing first-order tools. In a sense, then, this
paper contribution is \emph{not} to introduce yet another complexity
analysis methodology, but rather to show how complexity analysis can
be \emph{factored} into many subtasks, all but the last one being
program transformations. 


==> scratch.tex <==
\begin{lemma}\label{lem:narrow:helper}
  Consider a rewrite sequence 
  \[
  \fmain(\seq[n]{\dataone}) \rss[\atrsone] \ctx[\postwo]{\ctxone}[l\sigma] \rew[\atrsone] \ctx[\postwo]{\ctxone}[r\sigma] \rsl[\atrsone]{m} \termone 
  \tkom
  \]
  where $\dataone_j \in \DATA$ and $\termone$ is in normalform.
  Let $\atrsone_\funone \subseteq \atrsone$ be the rules defining $\funone$, i.e.\ those that are used in the construction of $\narrowings{\posone}{l \to r}$.
  
  If $\funone$ is sufficiently defined wrt. $\atrsone$ and 
  all rules in $\atrsone_\funone$ are redex-preserving, 
  then 
  \[
  \fmain(\seq[n]{\dataone}) \rss[\atrsone] \ctx[\postwo]{\ctxone}[l\sigma] \rew[\atrstwo] \ctx[\postwo]{\ctxone}[v\tau] \rsl[\atrsone]{n} \termone 
  \tkom
  \]
  for a rule $u \to v \in \narrowings{\posone}{l \to r}$, substitution $\ofdom{\tau}{\VS \to \Val[\CS_\TRSone]}$ and 
  $m \leqslant n + 1$. 
\end{lemma}
\begin{proof}
  We show the following three properties, from which the lemma follows.
  \begin{enumerate}
  \item 
    If $\funone$ is sufficiently defined wrt. $\atrsone$, 
    then $\ctx[\postwo]{\ctxone}[l\sigma] \rew[\atrstwo] \ctx[\postwo]{\ctxone}[v\tau]$ for some rule $u \to v \in \narrowings{\posone}{l \to r}$ and substitution 
    $\ofdom{\tau}{\VS \to \Val[\CS_\TRSone]}$; 
  \item 
    if $\termone$ is in normalform, then $\ctx[\postwo]{\ctxone}[v\tau] \rsl[\atrsone]{n} \termone$ for some $n \in \N$; and 
  \item 
    if the rules in $\atrsone_\funone$ are redex-preserving, then $m \leqslant n + 1$.
  \end{enumerate}
  % It suffices to consider the case where the applied rewrite rule is 
  % $l \to r \in \atrsone$. 
  Suppose $\funone$ is sufficiently defined wrt. $\atrsone$.
  Consider the subterm $\subtermAt{r}{\posone}\sigma$ of $r\sigma$.
  From the assumption on $\funone$, we see that $\subtermAt{r}{\posone}\sigma$
  is not a normalform of $\atrsone$ and thus reducible at the root, since $\atrsone$ is non-overlapping.
  Hence $\subtermAt{r}{\posone}\sigma$ matches the left-hand side $u'$ of a rule
  $u' \to v' \in \atrsone_\funone$.
  Wlog.\ we suppose that the rules in $\atrsone_\funone$ are variable disjoint with $r$, and thus, 
  the terms $\subtermAt{r}{\posone}$ and $u'$ are unifiable with an mgu $\mguone$, 
  which restricted to variables in $\subtermAt{r}{\posone}$ is at least as general as $\sigma$.
  Hence there is a substitution $\sigma_\mguone$, such that $\sigma(\varone) = \mguone(\varone)\sigma_\mguone$ for all variables $\varone$ in $\subtermAt{r}{\posone}$
  holds.
  By construction, there exists a rule $u \to v \in \narrowings{\posone}{l \to r}$ with $u = l\mguone$, obtained 
  by inlining $u' \to v'$ in $l \to r$. 
  Define $\tau$ as the extension of $\sigma_\mguone$, such that $\tau(\varone) = \sigma(\varone)$ for 
  variables $\varone$ occurring in $l$ but not in $\subtermAt{r}{\posone}$. 
  Then by definition $l\sigma = (l\mguone)\tau = u\tau$ and
  we conclude $\ctx[\postwo]{\ctxone}[l\sigma] = \ctx[\postwo]{\ctxone}[u\tau] \rew[\atrstwo] \ctx[\postwo]{\ctxone}[v\tau]$. 

  For the second property, suppose $\termone$ is in normalform and consider the reduction 
  $\ctx[\postwo]{\ctxone}[l\sigma] \rew[\atrsone] \ctx[\postwo]{\ctxone}[r\sigma] \rsl[\atrsone]{m} \termone$.
  %
  Lemma~\eref{l:narrow:irew}{ctx} gives a term $\termtwo$ in normalform and 
  $m_1,m_2 \in \N$ such that 
  $l\sigma \rew[\atrsone] r\sigma \rsl[\atrsone]{m_1} \termtwo$
  and $\ctx[\postwo]{\ctxone}[\termtwo] \rsl[\atrsone]{m_2} \termone$
  with $m = m_1 + m_2$. 
  Define $D \defsym \ctx[p]{r\mguone}[\hole]$ and $D_\tau \defsym D\tau$.
  Note that $r\sigma = (r\mguone)\tau$ holds by construction. 
  Thus $r\sigma = D_\tau[\subtermAt{(r\mguone)\tau}{\posone}]$.
  Since $\subtermAt{r}{\posone}\mguone = u' \mguone$, we have $\subtermAt{(r\mguone)\tau}{\posone} = (\subtermAt{r}{\posone}\mguone)\tau = (u'\mguone)\tau$
  thus overall, we can write $r\sigma = \ctx{D_\tau}[(u'\mguone)\tau]$.
  Likewise, using $v = \ctx{D}[v'\mguone]$, we can write $v\tau = \ctx{D_\tau}[(v'\mguone)\tau]$.
  Lemma~\ref{l:narrow:irew} thus yields for $r\sigma \rsl[\atrsone]{m_1} \termtwo$ an alternative derivation
  \[
  r\sigma = \ctx{D_\tau}[(u'\mguone)\tau] 
  \rsl[\atrsone]{n_1} \ctx{D_\tau}[u'\tau'] \rew[\atrsone] \ctx{D_\tau}[v'\tau'] 
  \rsl[\atrsone]{n_2} \termtwo
  \tkom
  \]
  with $m_1 = n_1 + n_2 + 1$.
  So clearly, 
  \[
  v\tau = \ctx{D_\tau}[(v'\mguone)\tau] \rsl[\atrsone]{n_1'} \ctx{D_\tau}[v'\tau'] 
  \rsl[\atrsone]{n_2} \termtwo
  \tkom
  \]
  as desired. 
  Overall, we obtain the derivation
  \[
  \ctxone[v\tau] \rsl[\atrsone]{n_1' + n_2} \ctxone[\termtwo] \rsl[\atrsone]{m_2} \termone \tkom
  \]
  of length $n \defsym n_1' + n_2 + m_2$.

  For the final property, it suffices to realise that for redex-preserving rules $u' \to v'$, 
  we additionally obtain $n_1 \leqslant n_1'$, 
  and hence $m = m_1 + m_2 = n_1 + n_2 + 1 + m_2 \leqslant n + 1$.
\end{proof}




  We first show 
  \begin{equation}
    \label{eq:narrowing:normalise}
    u\tau \rew[\atrstwo] v\tau \rss[\atrsone] \termtwo \IImp u\tau \rss[\atrsone] \termtwo\tkom
  \end{equation}
  where $u\tau$ occurs in a derivation from $\fmain(\seq[k]{\dataone})$, 
  $\ofdom{\tau}{\VS \to \Val[\CS_\TRSone]}$, 
  $\termtwo$ is in normalform and $u \to v \in \narrowings{\posone}{l \to r}$.
  Let $\mguone$ be the mgu with $u = l\mguone$. 
  Fix $u\tau \rew[\atrstwo] v\tau \rss[\atrsone] \termtwo$ as in the premise of \eqref{eq:narrowing:normalise}, 
  and thus there exists a normalised substitution $\ofdom{\tau'}{\VS \to \Val[\CS_\TRSone]}$ with 
  \[
  u\tau \rew[\atrstwo] v\tau \rss[\atrsone] v\tau' \rss[\atrsone] \termtwo 
  \tkom
  \]
  by Lemma~\eref{l:narrow:irew}{subst}.
  As in Lemma~\ref{lem:narrow:helper}, define $D \defsym \ctx[p]{r\mguone}[\hole]$ and $D_\tau \defsym D\tau$, 
  thus $(r\mguone)\tau = D_\tau[\subtermAt{(u'\mguone)\tau}{\posone}]$ 
  for the rule $u' \to v' \in \atrsone_\funone$ used in the construction of $u \to v$. 
  
  Then
  \[
  u\tau = (l\mguone)\tau \rew[\atrsone] (r\mguone)\tau = D_\tau[(u'\mguone)\tau] \rss[\atrsone] D_\tau[u'\tau'] \rew[\atrsone] D_\tau[v'\tau'] \tkom
  \]  
  for substitution $\ofdom{\tau'}{\VS \to \Val[\CS_\TRSone]$} since the symbol $\funone$ defined by $u' \to{} v'$ 
  is sufficiently defined wrt. $\atrsone$ and $\atrsone$ is non-ambigous.  
  
  






Naturally, there is no clear notion of a perfect strategy. After all, 
we are interested in non-trivial program properties. 
However, 
it is clear that any sensible strategy should at least 
(i) yield overall a transformation from \PCF\ to TRSs that is efficively computable, 
(ii)~not defeit its purpose by generating TRSs whose runtime-complexity 
is not at all in relation to the complexity of the analysed program, and
(iii)~not render current FOTs incapable on the resulting system. 

To address~(i), our tool uses rather naive but effectively computable approximations of 
usable rules and collecting semantics. We elaborate on our implementation of 
these techniques more in Section~\ref{s:timpl}.

Important also, the strategy employed in \hoca\ 
controls the growth of intermediate problems, avoiding an exponential blow-ups 
due to uncontrolled narrowing and instantiation. As a result, the number of 
basic transformations, such as narrowing and instantiation, is sufficiently 
bounded to be practical.
This strategy will be detailed in Section~\ref{s:strategy}.
Concerning~(ii), our strategy takes a conservative approach 
and only employes the methods of Section~\ref{s:simplify} if guaranteed to be
\emph{complexity-reflecting}. This way, the runtime-complexity function of the 
resulting TRS not only binds the runtime-complexity of the analysed program, 
but is also linearly related.
% For instance, using a notion dual to
% redex-preserving we ensure that calls in right-hand sides are not duplicated 
% by narrowing.
Points (iii)~is difficult, if not impossible, to formalize as it depends foremost 
on the methods employed in the back-end and the input program. To reduce the 
constraints needed to solve by FOTs, beside conrolling the size of the output, 
our strategy is designed to remove auxiliary functions, such as those introduced by 
the transformation of $\lambda$-abstractions, as much as possible. 
To this end, we agressively employ the rule-narrowing transformation. 


\paragraph{Rule-Narrowing:}
In contrast to its formalization, the implementation of rule-narrowing is in principle unspectacular. 
The main complication that arises in an automation of this technique is to decide where 
the transformation should be applied. Instead of hard-coding such a decision, our implementation 
\strat|narrow(P)| of rule-narrowing is parameterized by a predicate \strat|P| which decides, based on the 
current problem, rule $l \to r$ and position $\posone$, if it is \emph{sensible} to replace 
a rule $l \to r$ by its narrowings $\narrowings{\posone}{l \to r}$. This way, in our overall 
transformation we can use rule-narrowing in different states. 

%%%%%%%%%%%%
%% strategy

The strategy is displayed in a 
minimalistic language based on three operators. The first operator
$\transone_1 \scomp \transone_2$ denotes transformation 
composition $\transone_2 \cdot \transone_1$. 
Note that $\transone_1 \scomp \transone_2$ is inapplicable to an ATRS $\atrsone$ if 
either $\transone_1$ is inapplicable on $\atrsone$, or $\transone_2$ is inapplicable 
on the system generated by $\transone_1$. 
To override this behaviour, we use a combinator $\stry$ which
lifts a transformation $\transone$ to a total function:
\[
(\stry\ \transone) (\atrsone) \defsym 
\begin{cases}
  \transone(\atrsone) & \text{if $s_1(\atrsone)$ is defined,} \\
  \atrsone & \text{otherwise.}
\end{cases}
\]
Hence for instance $\stry\ \transone_1 \scomp \transone_2$ 
applies transformation $\transone_2$ independent on whether 
$\transone_1$ succeeds.
Exhaustive iteration of a transformation $\transone$ 
is thus expressible by the combinator $\sexhaustive$ satisfying
\[
  \sexhaustive\ s = \stry\ (s\ \scomp\ \sexhaustive\ s)
\tpkt
\]
Our final operator $\schoice$ implements a (left-biased) \emph{choice}: 
\[
(s_1 \schoice s_2) (\atrsone) \defsym 
\begin{cases}
  s_1(\atrsone) & \text{if $s_1(\atrsone)$ is defined} \\
  s_2(\atrsone) & \text{otherwise.}
\end{cases}
\]
It is not difficult to see that complexity-reflecting and 
complexity-preserving transformations are closed under 
the above operators. That is, starting from the basic 
transformations discussed in Section~\ref{s:timpl}, 
application of these operators results again in a transformation 
that is both complexity-reflecting and complexity-preserving. 

